Local Structure Theorems for Erdos Renyi Graphs and their Algorithmic Application

We analyze some local properties of sparse Erdos-Renyi graphs, where $d(n)/n$ is the edge probability. In particular we study the behavior of very short paths. For $d(n)=n^{o(1)}$ we show that $G(n,d(n)/n)$ has asymptotically almost surely (a.a.s.~) bounded local treewidth and therefore is a.a.s.~nowhere dense. We also discover a new and simpler proof that $G(n,d/n)$ has a.a.s.~bounded expansion for constant~$d$. The local structure of sparse Erdos-Renyi Gaphs is very special: The $r$-neighborhood of a vertex is a tree with some additional edges, where the probability that there are $m$ additional edges decreases with~$m$. This implies efficient algorithms for subgraph isomorphism, in particular for finding subgraphs with small diameter. Finally we note that experiments suggest that preferential attachment graphs might have similar properties after deleting a small number of vertices.

==> model_checking.tex <==
\subsection{Model-Checking}
\addressed[inline]{The proposed model-checking algorithm is the algorithm which is
well known for graphs which locally bounded tree-width (locally excluded
minors), for which now the expected running time is computed. I must strongly
criticise that the method is not put into context and is not attributed to the
original authors. Note that a simple algorithm follows also from earlier
analysis, e.g. that the expected number of short cycles in $\gnd$ is
constant. After removing these cycles and re-writing the formula to be checked
accordingly, we have a graph of local bounded tree-width and the algorithm for
locally bounded tree-width is applicable.}

\todo[inline]{Grohe hat gezeigt das man auf \ErRe model checking in $d(n)^{f(\varphi)}n$ machen kann wenn $d(n)=c$ ist. Peter glaubt das geht auch für $d(n)=n^{o(1)}$ durch, können wir das bestätigen oder vlt. ein Gegenbeispiel machen?\\

\bigskip
Selbst wenn es nicht durch geht ist es nicht linear fpt da die eingabegröße die Anzahl der Kanten sind. Neue Idee:

\smallskip
Berechne die $r-1$ Nachbarschaften von allen Knoten. benutze Feferman-Vaught um daraus die $r$ Nachbarschaften von allen Knoten zu bilden. Iteriere von $r=1$ bis $r=f(\varphi)$. Laufzeit: $f(\varphi) d(n) n$. Geht das alles durch?}

\label{sec:model_checking}

In this section we consider first-order model checking on random graphs.  If
we have a formula $\varphi$, we can test $G\models\varphi$ for general graphs
in $O(n^{|\varphi|})$ steps by using a naive algorithm, and in
$O(f(|\varphi|)n)$ steps in graphs of bounded expansion~\cite{DKT2013}. As we
have mentioned earlier, having \aas bounded expansion is not enough to
guarantee a fast expected runtime. For constant $d$ we can use
Theorem~\ref{thm:bounded_exp} and the associated probability bounds to do
efficient model checking by running the naive algorithm and the linear
algorithm in parallel to arrive at an expected running time of $O(n) +
\max\{n^{-2k},2^{-n^{2/3}}\} n^{|\varphi|} = O(n)$. 

Similarly, it is well known that the number of cycles of length $k$ in $\gndn$
is of order $d(n)^k$ (special case of Lemma~\ref{lem:num_h}). If $d(n)$ is
constant one can remove all short cycles and construct a formula which is
satisfiable on the locally tree-like graph if and only if the original formula
is satisfiable in the original graph. One can then use an fpt model checking
algorithm for locally bounded treewidth~\cite{locallyboundedtreewidth}. The
runtime of this technique, however, gets very large if $d(n)$ is not constant.
In this case, the formula blow-up depends on the (non-constant) number of
short cycles, therefore these techniques are already not fpt if for example
$d(n) = \log \log \log \log n$.

We will now show how to use our local structure results to get an expected
runtime of $O(d(n)^{g(|\varphi|)}n)$ for $\gndn$.
If $d(n)$ is polylogarithmic in $n$ the runtime is quasi-linear in $n$.
If $d=n^{o(1)}$ the runtime is $g(|\varphi|)n^{1+o(1)}$. 
We use a technique by Dawar, Grohe and
Kreutzer~\cite{DBLP:conf/lics/DawarGK07} which works as follows: We use
Gaifman's locality theorem~\cite{gaifman1982local} to break down $\varphi$
into local sentences that can be evaluated in small neighborhoods and combine
these solutions by constructing a scattered set.
\unsure[inline]{mention reference and runtime in introduction as well? verify!!}

Let $\psi^{N_r(x)}$ be the formula obtained from $\psi$ by requiring that all
quantifiers quantify only over the set $N_r(x)$.
\begin{lemma}\label{lem:fo-mcloc}
    Let $\phi$ be a formula of length $k$.
    For a vertex $v$ and a graph $G = \gndn$ one can decide whether $G \models \phi^{N_r(v)}(v)$ 
    in expected time $O\Big(f(k) \cdot |N_r(v)| + \frac{d(n)^{(2r+1)(k+1)}}{n}\Big)$.
\end{lemma}
\begin{proof}
    The algorithm distinguishes between two cases. The first case is that
    $N_r(v)$ contains at least $k+2$ more edges than vertices. In this case,
    we decide whether $G \models \phi$ by the naive $O(n^k)$ algorithm.
    Otherwise, the $r$-neighborhood of every vertex has treewidth at most
    $k+2$. By Courcelle's theorem~\cite{courcelle1990monadic}, one can decide
    whether $G \models \phi^{N_r(v)}(v)$ in time $ f(k) \; |N_r(v)|$.
    According to Lemma~\ref{lem:neighborhood_size}, the first case only occurs with probability at most $\big(\frac{d(n)^{2r+1}}{n}\big)^{k+1}$.
    The expected runtime is therefore bounded by
    $f(k) \; |N_r(v)| + \bigl(\frac{d(n)^{2r+1}}{n}\bigr)^{k+1} n^k$.
\end{proof}

A set of nodes is called an $r$-scattered set if the $r$-neighborhoods
of all pairs are disjoint.

\begin{lemma}\label{lem:scattered}
Let $G=(V,E)$ be a graph, $s,r>0$, and $R\subseteq V$.  Moreover, assume that 
every $(2sr)$-neighborhood in $G$ is a tree with at most $m$ additional
edges.  The average size of all $(2sr)$-neighborhoods is~$w$.
Then we can find out in time $O(g'(m,s,r)w|V|)$ whether $R$ contains an
$r$-scattered set of size~$s$, where $g'$ is some computable function.
\end{lemma}

\begin{proof}
We look at all vertices in $R$ and find greedily an $r$-scattered
subset~$S$.  This takes time at most $|R|w$.  It $|S|\geq s$ we are
done.  Otherwise all nodes from $R$ have distance at most $2r$
from~$S$.  Now look at the graph $H=G[F]$, where $F$ is the set of all
edges in all $2r$-neighborhoods of all nodes in~$S$.  Obviously, $H$
contains \emph{all} nodes from~$R$.  Moreover, $H$'s components have a
diameter of at most~$2sr$.  It is easy to construct $H$ within the given
time bound.  Because every component of $H$ is a tree with at most $m$
additional edges, the treewidth of $H$ is at most $m+1$ and we can
easily construct a tree decomposition of this width.  Using
Courcelle's theorem we can find an $r$-scattered set of maximal size
in $H$, because we can express it as an MSO-formula whose length
depends only on $r$ and~$s$.
\end{proof}

\begin{lemma}\label{lem:fo-mc}
    There exists a function $g$ such that 
    for a fixed FO-sentence $\varphi$, one can do FO-model-checking in $\gndn$ in time $O(d(n)^{g(|\varphi|)} n)$.
\end{lemma}
\begin{proof}
    By Gaifman locality, the sentence $\varphi$ is equivalent to a Boolean
    combination of basic $r$-local sentences $\psi_1, \dots \psi_l$. 
    If we evaluate $\psi_1,\dots,\psi_l$ we can easily compute
    whether $G \models \varphi$. 
    Let $\delta(x,y) > r$ be the first order formula denoting that the distance
    between $x$ and $y$ is greater than $r$. 
    A $r$-local sentence $\psi$ has the
    structure
    $$
    \psi = \exists x_1 \dots \exists x_s \Big(\bigwedge_{i\neq j} 
    \delta(x_i,x_j) > 2r \wedge \bigwedge_i \phi^{N_r(x_i)}(x_i) \Big).
    $$
    %Let $t$ be the maximal number of $\exists$ quantifiers in any of these $r$-local sentences.
    Using Lemma~\ref{lem:fo-mcloc}, Lemma~\ref{lem:neighborhood_size} and linearity of expectation, 
    we can decide for each vertex $v \in V$ whether $G \models \phi^{N_r(v)}(v)$ in expected time
    $$
    \sum_{v \in V} O\biggl(f(|\psi|) \cdot \E[|N_r(v)|] +
    \frac{d(n)^{(2r+1)(|\psi|+1)}}{n}\biggr) =  O\big(f(|\psi|) d(n)^r n  + d(n)^{(2r+1)(|\psi|+1)}\big)
    $$
    and color these vertices red.
    It holds that $G \models \psi$ iff there exists an $r$-scattered set of
    $s$ red vertices.
    Before we try to find out whether such a set exists, we test
    whether every $(2rs)$-neighborhood in $G$ is a tree with at most
    $m=|\varphi|+1$ additional edges.  By Lemma~\ref{lem:lcycles} this test
    fails with a probability of at most $d(n)^{4rs}(d(n)^{4rs+1}/n)^m$, in which
    case we can check $G\models\varphi$ in $O(n^{|\varphi|})$ time by the
    naive algorithm without hurting the expected runtime.
    Otherwise, we can check whether such a set exists using
    Lemma~\ref{lem:scattered} in time $O(g'(m,s,r)d(n)^rn)$.

    Therefore we can decide whether $\psi$ holds in time
    $O(f(|\psi|) d(n)^r n  + d(n)^{(2r+1)(|\psi|+1)})$.
    We need to do this computation $l$ times. 
    The values $l$, $r$, $s$, and $|\psi|$ depend only on $\varphi$, therefore there exists a function
    $g$ such that the expected runtime is bounded by $O(d(n)^{g(|\varphi|)}n)$.
\end{proof}
%\todo[inline]{
%What implications does this have if $d=\log n$, $d < 1$, $d > 1$ or $d=1$?
%}
